Cloning Games, Black Holes and Cryptography

In this work, we introduce a new toolkit for analyzing cloning games, a notion that captures stronger and more quantitative versions of the celebrated quantum no-cloning theorem. This framework allows us to analyze a new cloning game based on binary phase states. Our results provide evidence that these games may be able to overcome important limitations of previous candidates based on BB84 states and subspace coset states: in a model where the adversaries are restricted to making a single oracle query, we show that the binary phase variant is $t$-copy secure when $t=o(n/\log n)$. Moreover, for constant $t$, we obtain the first optimal bounds of $O(2^{-n})$, asymptotically matching the value attained by a trivial adversarial strategy. We also show a worst-case to average-case reduction which allows us to show the same quantitative results for the new and natural notion of Haar cloning games. Our analytic toolkit, which we believe will find further applications, is based on binary subtypes and uses novel bounds on the operator norms of block-wise tensor products of matrices. To illustrate the effectiveness of these new techniques, we present two applications: first, in black-hole physics, where our asymptotically optimal bound offers quantitative insights into information scrambling in idealized models of black holes; and second, in unclonable cryptography, where we (a) construct succinct unclonable encryption schemes from the existence of pseudorandom unitaries, and (b) propose and provide evidence for the security of multi-copy unclonable encryption schemes.

==> unitary-designs.tex <==
\section{Mixed Unitary Designs}
%%%%%%%%%%%%

In this section, we'll introduce a more general version of a unitary $r$-design which also handles inverses.

\subsection{Vectorization Formalism.}
For a linear operator $\boldsymbol{\Lambda} \in \mathrm{L}(\mathbb{C}^d)$, we consider the vectorization $\mathrm{vec}: \mathrm{L}(\mathbb{C}^d) \rightarrow (\mathbb{C}^d)^{\ot 2}$ such that
$$
\boldsymbol{\Lambda}  = \sum_{i,j \in [d]} \Lambda_{(i,j)} \ket{i}\hspace{-1mm}\bra{j} \quad \mapsto \quad \mathrm{vec}(\boldsymbol{\Lambda} ) :=\kett{\boldsymbol{\Lambda} } = \sum_{i,j \in [d]} \Lambda_{(i,j)} \ket{i} \otimes \ket{j}.
$$
We're also going to use the so-called ABC-rule~\cite{Mele2024introductiontohaar}: for any linear operators $\vec{A,B,C} \in \mathrm{L}(\mathbb{C}^d)$,
$$
\kett{\vec{ABC}} = (\vec A \otimes \vec C^\intercal) \kett{\vec B}.
$$

\subsection{Non-Adaptive Mixed Unitary Designs}

\begin{definition}[Mixed-Adjoint Moment Operator]
Let $\nu$ be an ensemble of unitary operators over $\mathbb{C}^d$. Then, we define the mixed-adjoint $(p,q)$-moment operator $\algo M_{\nu, \mathsf{adj}}^{(p,q)} : \mathrm{L}(\mathbb{C}^d) \rightarrow \mathrm{L}(\mathbb{C}^d)$ by
$$
\algo M_{\nu, \mathsf{adj}}^{(p,q)}(\vec O) := \underset{U \sim \nu}{\mathbb{E}}\left[(U^{\otimes p} \otimes (U^\dag)^{\otimes q}) \vec O (U^{\otimes p} \otimes  (U^\dag)^{\otimes q})^\dag \right] 
$$
for a linear operator $\vec O \in \linear((\CC^d)^{\otimes (p+q)})$. Similarly, we let $\algo M_{\algo U_d, \mathsf{adj}}^{(p,q)}$ denote the mixed-adjoint $(p,q)$-moment operator with respect to the Haar measure over the unitary group $\algo U_d$.
\end{definition}

\begin{definition}[Non-Adaptive Mixed Unitary $(p,q)$-Design]
Let $\nu$ be an ensemble of unitary operators over $\mathbb{C}^d$. Then, $\nu$ is a (non-adaptive) unitary $(p,q)$-design if, for every $\vec O \in \linear((\CC^d)^{\otimes (p+q)})$,
$$
\underset{U \sim \nu}{\mathbb{E}}\left[(U^{\otimes p} \otimes (U^\dag)^{\otimes q}) \vec O (U^{\otimes p} \otimes  (U^\dag)^{\otimes q})^\dag \right] = \underset{U \sim \algo U_d}{\mathbb{E}}\left[(U^{\otimes p} \otimes (U^\dag)^{\otimes q}) \vec O (U^{\otimes p} \otimes  (U^\dag)^{\otimes q})^\dag \right].
$$
\end{definition}

Note that a unitary $r$-design is a special case of the above definition.

\begin{definition}[Non-Adaptive Unitary $r$-Design]
Let $\nu$ be an ensemble of unitary operators over $\mathbb{C}^d$. Then, $\nu$ is a (non-adaptive) unitary $r$-design if it is a (non-adaptive) unitary $(r,q)$-design for $q=0$.
\end{definition}

We show the following equivalence in terms of the vectorized mixed moment operator.

\begin{lemma}\label{lem:equiv-mixed-design}
A unitary ensemble $\nu$ over $\mathbb{C}^d$ is a (non-adaptive) unitary $(p,q)$-design if and only if
$$
\underset{U \sim \nu}{\mathbb{E}}\left[U^{\otimes p} \otimes (U^\dag)^{\otimes q}  \otimes  \bar{U}^{\otimes p} \otimes  (U^\intercal)^{\otimes q} \right] = \underset{U \sim \algo U_d}{\mathbb{E}}\left[U^{\otimes p} \otimes (U^\dag)^{\otimes q}  \otimes  \bar{U}^{\otimes p} \otimes  (U^\intercal)^{\otimes q}\right].
$$
\end{lemma}
\begin{proof} Suppose that $\nu$ is a unitary $(p,q)$-design. Then, for all $\vec O \in \linear((\CC^d)^{\otimes (p+q)})$, it holds that
$$
\algo M_{\nu,\mathsf{adj}}^{(p,q)}(\vec O) =\algo M_{\algo U_d,\mathsf{adj}}^{(p,q)}(\vec O).
$$
By applying the vectorization $\mathrm{vec}: \mathrm{L}((\CC^d)^{\otimes (p+q)}) \rightarrow ((\CC^d)^{\otimes (p+q)})^{\ot 2}$  on both sides, we get
$$
\kett{\algo M_{\nu,\mathsf{adj}}^{(p,q)}(\vec O)} = \kett{\algo M_{\algo U_d,\mathsf{adj}}^{(p,q)}(\vec O)}.
$$
By linearity and the $ABC$-rule for $\mathrm{vec}(\cdot)$, this is equivalent to
$$
\underset{U \sim \nu}{\mathbb{E}}\left[U^{\otimes p} \otimes (U^\dag)^{\otimes q}  \otimes  \bar{U}^{\otimes p} \otimes  (U^\intercal)^{\otimes q} \right]\kett{\vec O} = \underset{U \sim \algo U_d}{\mathbb{E}}\left[U^{\otimes p} \otimes (U^\dag)^{\otimes q}  \otimes  \bar{U}^{\otimes p} \otimes  (U^\intercal)^{\otimes q} \right] \kett{\vec O}.
$$
Because $\mathrm{vec}(\cdot)$ is a bijection between $\mathrm{L}((\CC^d)^{\otimes (p+q)}) $ and $((\CC^d)^{\otimes (p+q)})^{\ot 2}$, the operators above must be identical on the entire vector space $((\CC^d)^{\otimes (p+q)})^{\ot 2}$. The converse statement can be shown analogously.
\end{proof}

\begin{lemma}\label{lem:t-design-to-mixed}
A unitary $r$-design $\nu$ is a mixed unitary $(p,q)$-design for any $p,q$ with $r=p+q$.
\end{lemma}
\begin{proof}
Let $r=p+q$. According to \Cref{lem:equiv-mixed-design}, it suffices to show that $\nu$ satisfies
$$
\underset{U \sim \nu}{\mathbb{E}}\left[U^{\otimes p} \otimes (U^\dag)^{\otimes q}  \otimes  \bar{U}^{\otimes p} \otimes  (U^\intercal)^{\otimes q}\right] = \underset{U \sim \algo U_d}{\mathbb{E}}\left[U^{\otimes p} \otimes (U^\dag)^{\otimes q}  \otimes  \bar{U}^{\otimes p} \otimes  (U^\intercal)^{\otimes q} \right].
$$
By inserting the partial transpose with respect to the 2nd and 4th system, this is equivalent to
$$
\underset{U \sim \nu}{\mathbb{E}}\left[U^{\otimes p} \otimes \bar{U}^{\otimes q}  \otimes  \bar{U}^{\otimes q} 
\otimes U^{\otimes p} \right]^{\mathsf{T}_{2,4}} = \underset{U \sim \algo U_d}{\mathbb{E}}\left[U^{\otimes p} \otimes \bar{U}^{\otimes q}  \otimes  \bar{U}^{\otimes q} 
\otimes U^{\otimes p}\right]^{\mathsf{T}_{2,4}}.
$$
After inserting a $\mathsf{SWAP}$ between the 2nd and 4th system via $\mathbb{F}_{2,4}$, it is also equivalent to showing that
$$
\left[\mathbb{F}_{2,4}^\dag\underset{U \sim \nu}{\mathbb{E}}\left[U^{\otimes p}  \otimes  U^{\otimes q} \otimes  \bar{U}^{\otimes p} \otimes \bar{U}^{\otimes q}  \right]\mathbb{F}_{2,4}\right]^{\mathsf{T}_{2,4}}= \left[\mathbb{F}_{2,4}^\dag\underset{U \sim \algo U_d}{\mathbb{E}}\left[U^{\otimes p}  \otimes  U^{\otimes q} \otimes  \bar{U}^{\otimes p} \otimes \bar{U}^{\otimes q}  \right]\mathbb{F}_{2,4}\right]^{\mathsf{T}_{2,4}}.
$$
By assumption, $\nu$ is a unitary $r$-design for $r=p+q$, and hence it holds that 
$$
\underset{U \sim \nu}{\mathbb{E}}\left[U^{\otimes p}  \otimes  U^{\otimes q} \otimes  \bar{U}^{\otimes p} \otimes \bar{U}^{\otimes q}  \right] = \underset{U \sim \algo U_d}{\mathbb{E}}\left[U^{\otimes p}  \otimes  U^{\otimes q} \otimes  \bar{U}^{\otimes p} \otimes \bar{U}^{\otimes q}  \right]
$$
which yields the desired equality from before.
\end{proof}



\subsection{Adaptive Mixed Unitary Designs}

In this section, we generalize the notion of mixed unitary designs to algorithms which may query a unitary (and possibly its inverse) adaptively, rather than in parallel.

\begin{definition}[Adaptive Mixed Unitary $(p,q)$-Design]
Let $\nu$ be an ensemble of unitary operators over $\mathbb{C}^d$. Then, $\nu$ is an adaptive unitary $(p,q)$-design if, for every single-bit output (possibly adaptive) quantum algorithm $\algo A$ making at most $p$ many queries to a unitary and $q$ many queries to its adjoint,
$$
\Pr\left[ 1 \leftarrow \algo A^{U,U^\dag }(1^{\lceil \log d \rceil}) \, : \, U \sim \nu \right] = \Pr\left[ 1 \leftarrow \algo A^{U,U^\dag }(1^{\lceil \log d \rceil}) \, : \, U \sim \algo U_d \right].
$$
We say that $\nu$ is an adaptive mixed unitary $t$-design if the property above holds for any adaptive quantum query algorithm $\algo A$ which submits no more than $t$ queries to either $U$ or $U^\dag$.
\end{definition}

We now show that an (exact) non-adaptive mixed unitary $r$-design is automatically also an (exact) adaptive mixed unitary $r$-design. In the approximate case, this conversion incurs an exponential blow-up.

\begin{theorem}
Any exact non-adaptive unitary $r$-design is also an exact adaptive mixed unitary $r$-design.    
\end{theorem}
\begin{proof}
Let $\nu$ be a non-adaptive unitary $r$-design over $\mathbb{C}^d$. Suppose that $\algo A^{U,U^\dag}(1^{\lceil \log d \rceil})$ is an adaptive $r$-query quantum algorithm that makes $p$ many queries to $U$ and $q$ queries to $U^\dag$, for $U \in \algo U_d$ and $r=p+q$.

The idea is to use quantum gate teleportation. Specifically, we show that, for any $U \in \algo U_d$, there exists a non-adaptive algorithm $\algo B^{U,U^\dag}(1^{\lceil \log d \rceil})$ that makes $p$ many parallel queries to $U$ and $q$ many parallel queries to $U^\dag$ such that
$$
\Pr\left[ 1 \leftarrow \algo A^{U,U^\dag }(1^{\lceil \log d \rceil})  \right] = d^{2(p+q)} \Pr\left[ 1 \leftarrow \algo B^{U,U^\dag }(1^{\lceil \log d \rceil}) \right].
$$
Because $\nu$ is a non-adaptive unitary $r$-design, we know from \Cref{lem:t-design-to-mixed} that $\nu$ is also mixed unitary $(p,q)$-design. Putting everything together, we get that
\begin{align*}
\Pr\left[ 1 \leftarrow \algo A^{U,U^\dag }(1^{\lceil \log d \rceil}) \, : \, U \sim \nu \right] &= d^{2(p+q)}\Pr\left[ 1 \leftarrow \algo B^{U,U^\dag }(1^{\lceil \log d \rceil}) \, : \, U \sim \nu \right]\\
&= d^{2(p+q)}\Pr\left[ 1 \leftarrow \algo B^{U,U^\dag }(1^{\lceil \log d \rceil}) \, : \, U \sim \algo U_d \right]\\
&=\Pr\left[ 1 \leftarrow \algo A^{U,U^\dag }(1^{\lceil \log d \rceil}) \, : \, U \sim \algo U_d \right].    
\end{align*}
This proves the claim.
\end{proof}

%%%%%%%%%%

